Multi-Microphone Speaker Separation by Spatial Regions

We consider the task of region-based source separation of reverberant multi-microphone recordings. We assume pre-defined spatial regions with a single active source per region. The objective is to estimate the signals from the individual spatial regions as captured by a reference microphone while retaining a correspondence between signals and spatial regions. We propose a data-driven approach using a modified version of a state-of-the-art network, where different layers model spatial and spectro-temporal information. The network is trained to enforce a fixed mapping of regions to network outputs. Using speech from LibriMix, we construct a data set specifically designed to contain the region information. Additionally, we train the network with permutation invariant training. We show that both training methods result in a fixed mapping of regions to network outputs, achieve comparable performance, and that the networks exploit spatial information. The proposed network outperforms a baseline network by 1.5 dB in scale-invariant signal-to-distortion ratio.

==> Multi-Microphone Speaker Separation by Spatial Regions-2/figures/source1.tex <==

\definecolor{darkslategray38}{RGB}{234,234,242}
\definecolor{lavender234234242}{RGB}{234,234,242}
\definecolor{steelblue31119180}{RGB}{234,234,242}

\begin{axis}[
axis background/.style={fill=lavender234234242},
axis line style={white},
tick align=outside,
x grid style={white},
xmajorgrids,
xmajorticks=false,
xmin=1, xmax=1.5,
y grid style={white},
ymajorgrids,
ymajorticks=false,
ymin=0.25, ymax=0.75,
ytick style={color=darkslategray38},
mark color=orange,
]
\addplot [
height=1cm,
width=1cm,
color=black,
  mark=*,
  only marks,
  mark options={fill=white},
  scatter/@pre marker code/.append style={/tikz/mark size=\perpointmarksize},
  visualization depends on={\thisrow{sizedata} \as\perpointmarksize},
]
table[meta=label]{%
x  y  sizedata label
1.30769809 0.28769062 4.7194911794179895 a
1.04238692 0.41650123 5.5474817226236866 a
1.07357845 0.2648235 5.641895835477563 a
1.30359685 0.53297232 4.065459869851374 a
1.45465798 0.27990461 4.505452788852531 a
1.16758733 0.57877589 4.006257839457674 a
1.29957739 0.39556262 4.504599115397216 a
1.07628639 0.53420481 5.1624359175130685 a
1.39436507 0.40841806 4.1352405247271955 a
1.49604073 0.72940088 1.7841241161527712 a
};
\end{axis}



==> figures/source1.tex <==

\definecolor{darkslategray38}{RGB}{234,234,242}
\definecolor{lavender234234242}{RGB}{234,234,242}
\definecolor{steelblue31119180}{RGB}{234,234,242}

\begin{axis}[
axis background/.style={fill=lavender234234242},
axis line style={white},
tick align=outside,
x grid style={white},
xmajorgrids,
xmajorticks=false,
xmin=1, xmax=1.5,
y grid style={white},
ymajorgrids,
ymajorticks=false,
ymin=0.25, ymax=0.75,
ytick style={color=darkslategray38},
mark color=orange,
]
\addplot [
height=1cm,
width=1cm,
color=black,
  mark=*,
  only marks,
  mark options={fill=white},
  scatter/@pre marker code/.append style={/tikz/mark size=\perpointmarksize},
  visualization depends on={\thisrow{sizedata} \as\perpointmarksize},
]
table[meta=label]{%
x  y  sizedata label
1.30769809 0.28769062 4.7194911794179895 a
1.04238692 0.41650123 5.5474817226236866 a
1.07357845 0.2648235 5.641895835477563 a
1.30359685 0.53297232 4.065459869851374 a
1.45465798 0.27990461 4.505452788852531 a
1.16758733 0.57877589 4.006257839457674 a
1.29957739 0.39556262 4.504599115397216 a
1.07628639 0.53420481 5.1624359175130685 a
1.39436507 0.40841806 4.1352405247271955 a
1.49604073 0.72940088 1.7841241161527712 a
};
\end{axis}


